A Tutorial on Neural Networks and Gradient-free Training

This paper presents a compact, matrix-based representation of neural networks in a self-contained tutorial fashion. Specifically, we develop neural networks as a composition of several vector-valued functions. Although neural networks are well-understood pictorially in terms of interconnected neurons, neural networks are mathematical nonlinear functions constructed by composing several vector-valued functions. Using basic results from linear algebra, we represent a neural network as an alternating sequence of linear maps and scalar nonlinear functions, also known as activation functions. The training of neural networks requires the minimization of a cost function, which in turn requires the computation of a gradient. Using basic multivariable calculus results, the cost gradient is also shown to be a function composed of a sequence of linear maps and nonlinear functions. In addition to the analytical gradient computation, we consider two gradient-free training methods and compare the three training methods in terms of convergence rate and prediction accuracy.

==> Sections/NN.tex <==


\section{Neural Networks}
\label{sec:neural_networks}

This section presents a compact matrix-based representation of neural networks.
% A neural network is composed of several \textit{neural layers}, and each neural layer is composed of several \textit{neurons}.
% 
Specifically, in this section, we write neurons and neural layers as mathematical functions and construct neural networks as composition of several neural layers. 

A \textit{neuron} is the most basic component of a neural network. 
% 
Mathematically, the input to a neuron is a real-valued vector, and its output is a scalar. 

\begin{definition} \rm
A \textit{neuron} is a real-valued function 
\begin{align}
    n \colon \BBR^{l_x} \times \BBR^{l_x+1} \mapsto \BBR
\end{align}
constructed by the composition of a nonlinear function $\sigma \colon \BBR \mapsto \BBR$ and a bi-linear function $\SL \colon \BBR^{l_x} \times \BBR^{l_x+1} \mapsto \BBR,$ that is, $n = \sigma \circ \SL. $
% that is composed of a bi-linear function $\SL \colon \BBR^{l_x} \times \BBR^{l_x+1} \mapsto \BBR$ and a nonlinear function $\sigma \colon \BBR \mapsto \BBR$, that is, $n = \sigma \circ \SL. $
% 
The output of a neuron is thus computed as
\begin{align}
    n(x,\theta)
        &=
            \sigma (\SL(x,\theta) ),
\end{align}
where $\SL(x,\theta) = \matl x^\rmT & 1 \matr \theta.$
Defining $\chi \isdef \matl x^\rmT & 1 \matr^\rmT \in \BBR^{l_x+1}$, it follows that $\SL(x,\theta) = \chi^\rmT \theta.$
The vector $\theta \in \BBR^{l_x+1}$ is called the \textit{neuron gain}. 
% 
The nonlinear function $\sigma$ is also called the \textit{activation function}. 

An example of an activation function is the sigmoid function 
\begin{align}
    \sigma(z)
        =
            \frac{1}
            {1+e^{-z}}.
\end{align}
Alternatively, softmax, linear, harmonic, logarithmic, ReLU, and other functions are also used as the activation function \cite{sharma2017activation}. 
A neuron is shown in Figure \ref{fig:neuron}.
% \begin{align}
%     n:\BBR^{l_x} \times \BBR^{l_x} &\to \BBR,
%     \nn \\
%     n(\theta, x) 
%         &=
%             \frac{1}
%             {1+e^{-\theta^\rmT x}}.
% \end{align}

\end{definition}


\begin{figure}
    \centering
    \subfloat[Anatomy of a neuron.]
    {
    \centering
    % \resizebox{\columnwidth}{!}
    {
    \begin{tikzpicture}[auto, node distance=2cm,>=latex',text centered]
    
        \draw [draw=black, fill = gray, opacity=0.25] (-2.25,-1.5) rectangle (3.5,1.5);
        \node at (-3,0) (input) {$x$};
        \node [smallblock, right = 3 em of input,text width=1.6cm] (bilinear) {Bilinear function};
        % , minimum height=3em, text width=1.6cm
        
        \node [smallblock, right = 3 em of bilinear,text width=1.6cm] (activation) {Activation function};
        % \node at {(Plant)+(3,0)}  (output) {$y$};
        \node[right = 3 em of activation] (output) {$y$};
        
        \draw[->] (input) -- (bilinear);
        \draw[->] (bilinear) -- (activation);
        \draw[->] (activation) -- (output);
        % \draw[->] (sum) -- node[xshift = 0em, yshift = .2em]{$e$} (Controller);
        % \draw[->] (Controller)-- node[xshift = 0em, yshift = .2em]{$u$} (Plant);
        % \draw[->] (Plant) -- (output);
        % \draw[->] (Plant.east) -- +(1,0) -- +(+1,-1.5)
        %             -| (sum.south);
        \draw[->] (bilinear.north)+(0,0.5) node[xshift = 0em, yshift = +0.5em]{$\theta$} -- (bilinear.north);
        
        
    \end{tikzpicture}
    }
    }
    \\ 
    \subfloat[Simplified representation of a neuron.]
    {
    \centering
    % \resizebox{\columnwidth}{!}
    {
    \begin{tikzpicture}[auto, node distance=2cm,>=latex',text centered]
        \node at (-3,0) (input) {$x$};
        \node [smallblock, right = 3 em of input,text width=1.6cm] (Neuron) {Neuron};
        % , minimum height=3em, text width=1.6cm
        
        \node[right = 3 em of Neuron] (output) {$y$};
        
        \draw[->] (input) -- (Neuron);
        \draw[->] (Neuron) -- (output);
        \draw[->] (bilinear.north)+(0,0.5) node[xshift = 0em, yshift = +0.5em]{$\theta$} -- (bilinear.north);
        
        % \node at (0,-1.4) {};
    \end{tikzpicture}
    }
    }
    \caption{A neuron.}
    \label{fig:neuron}
\end{figure}

A \textit{neural layer} is composed of several neurons. 
The output of the neural layer is a vector whose dimension is equal to the number of neurons in the neural layer. 
Note that each neuron receives the same input.
\begin{definition}
\rm
Let $l_\theta \isdef l_x+1.$
An \textit{$\ell-$dimensional neural layer} is a vector-valued function 
\begin{align}
    N:\BBR^{l_x} \times \BBR^{l_\theta \times \ell} \mapsto  \BBR^{\ell},
\end{align}
constructed by $\ell$ neurons. 
The output of a neural layer is computed as
\begin{align}
    N(x, \Theta) 
        =
            \matl
                n (x, \Theta e_1) \\
                \vdots \\
                n (x,\Theta e_\ell )
            \matr,
\end{align}
% where each neuron $n_i$ is parameterized by the vector $\theta_i \in \BBR^{l_x}.$
where $\Theta \isdef \matl \theta_1 & \ldots & \theta_{\ell} \matr \in \BBR^{l_\theta \times \ell}$ is the \textit{neural layer gain matrix}
and for $i = \{1, \ldots, \ell\},$ $e_i$ is the $i$th column of the $\ell \times \ell$ identity matrix. 
% $I_\ell$
Note that the neural layer 
% is parameterized by the matrix $\Theta \isdef \matl \theta_1 & \ldots \theta_{l_y} \matr \in \BBR^{l_x \times l_y},$ and thus 
can be written as
% 
\begin{align}
    N(x,\Theta) 
        =
            \matl
                \sigma(\SL(x, \Theta e_1) \\
                \vdots \\
                \sigma(\SL(x, \Theta e_{l_y})
            \matr.
\end{align}

\end{definition}

A neural layer is shown in Figure \ref{fig:neural_layer}.

\begin{figure}[h]
    \centering
    \subfloat[Anatomy of a neural layer.]
    {
    \centering
    % \resizebox{\columnwidth}{!}
    {
    \begin{tikzpicture}[auto, node distance=2cm,>=latex',text centered]
        \draw [draw=black, fill = gray, opacity=0.25] (-2.5,-2.75) rectangle (3.25,3.25);
        
        \node at (-3,0) (input) {$x$};
        \node [smallblock, right = 3 em of input,text width=1.6cm] (Neuron) {Neuron $j$};
        
        \node [smallblock, above = 3 em of Neuron,text width=1.6cm] (Neuron_1) {Neuron $1$};
        
        \node [smallblock, below = 3 em of Neuron,text width=1.6cm] (Neuron_ell) {Neuron $\ell$};
        
        \node [smallblock, right = 3 em of Neuron,text width=1.6cm] (Vec) {Vectorize};
        
        % , minimum height=3em, text width=1.6cm
        
        
        % \node at {(Plant)+(3,0)}  (output) {$y$};
        \node[right = 3 em of Vec] (output) {$y$};
        
        \draw[->] (input) -- (Neuron);
        \draw[->] (input) -| +(0.75,1) |- (Neuron_1.180);
        \draw[->] (input) -| +(0.75,1) |- (Neuron_ell.180);
        \draw[->] (Neuron) -- (Vec);
        \draw[->] (Neuron_1) -| +(1.5,0) |- (Vec.165);
        \draw[->] (Neuron_ell) -| +(1.5,0) |- (Vec.195);
        \draw[->] (Vec) -- (output);
        % \draw[->] (sum) -- node[xshift = 0em, yshift = .2em]{$e$} (Controller);
        % \draw[->] (Controller)-- node[xshift = 0em, yshift = .2em]{$u$} (Plant);
        % \draw[->] (Plant) -- (output);
        % \draw[->] (Plant.east) -- +(1,0) -- +(+1,-1.5)
        %             -| (sum.south);
        
        \draw[->] (Neuron_1.north)+(0,0.5) node[xshift = -0.75em, yshift = -0.5em]{$\theta_1$} -- (Neuron_1.north);
        \draw[->] (Neuron.north)+(0,0.5) node[xshift = -0.75em, yshift = -0.5em]{$\theta_j$} -- (Neuron.north);
        \draw[->] (Neuron_ell.north)+(0,0.5) node[xshift = -0.75em, yshift = -0.5em]{$\theta_\ell$} -- (Neuron_ell.north);
        
    \end{tikzpicture}
    }
    }
    \\ 
    \subfloat[Simplified representation of a neural layer.]
    {
    \centering
    % \resizebox{\columnwidth}{!}
    {
    \begin{tikzpicture}[auto, node distance=2cm,>=latex',text centered]
        \node at (-3,0) (input) {$x$};
        \node [smallblock, right = 3 em of input,text width=1.6cm] (Neuron) {Neural Layer};
        % , minimum height=3em, text width=1.6cm
        
        \node[right = 3 em of Neuron] (output) {$y$};
        
        \draw[->] (input) -- (Neuron);
        \draw[->] (Neuron) -- (output);
        \draw[->] (bilinear.north)+(0,0.5) node[xshift = 0em, yshift = +0.5em]{$\Theta$} -- (bilinear.north);
        
        % \node at (0,-2.65) {};
    \end{tikzpicture}
    }
    }
    \caption{A neural layer.}
    \label{fig:neural_layer}
\end{figure}

% Note that a neuron layer is parameterized by $l_x l_y$ parameters. 
% Furthermore, a neuron layer with one output is a neuron. 


% \begin{definition}
% \rm
% A \textit{neuron layer} is a function $N:\BBR^{l_x \times l_y} \times \BBR^{l_x} \to \BBR^{l_y}$ such that
% \begin{align}
%     N(\Theta, x) 
%         =
%             \matl{c}
%                 n_1 (\Theta e_1, x) \\
%                 \vdots \\
%                 n_{l_y} (\Theta e_{l_y}, x)
%             \matr.
% \end{align}
% Note that a neuron layer is parameterized by $l_x l_y$ parameters. 
% Furthermore, a neuron layer with one output is a neuron. 

% \end{definition}

A \textit{neural network} is composed of several neural layers. Each neural layer can have an arbitrary number of neurons.

\begin{definition}
\rm 
An \textit{$n$-layer neural network} is a vector-valued function 
\begin{align}
    NN \colon 
\BBR^{l_{x}} \times 
\BBR^{l_{\theta_1} \times \ell_1} \times 
\cdots \times
\BBR^{l_{\theta_n} \times \ell_n} \times 
\BBR^{l_{\ell_n} \times l_y} 
\mapsto \BBR^{l_y},
\end{align}
constructed by the composition of $n$ neural layers, 
where, for each $i \in \{1, 2, \ldots, n\},$ $l_{x_1} = l_x$,  
$l_{x_{i+1}} \isdef \ell_i,$ and 
$l_{\theta_i} \isdef l_{x_i}+1.$
% that is composed of $n$ neural layers,
Note that the $i$th neural layer $N_i$ is $\ell_i$ dimensional  
and the final layer is typically  linear, that is, 
\begin{align}
    NN
        &= 
            S \circ N_n \circ N_{n-1} \circ \ldots \circ N_1,
\end{align}
where $S$ is a linear map. 
The output of the neural network is computed as
\begin{align}
    NN(x, &\Theta_1, \ldots, \Theta_n,\Theta_{n+1})
        \nn \\
        = 
            \Theta_{n+1} &N_n ( N_{n-1} (\ldots ( N_1(x,\Theta_1)),\Theta_{n-1} )\Theta_n ),
\end{align}


% 

% 
% composition of neural layers. 
\end{definition}

% Note that the $i$th layer in the neural network is $N_i.$
The output of a neural network can be computed using a recursive formula as shown below. 
By denoting the input and the output of the $i$th neural layer by $x_i$ and $x_{i+1},$ it follows that, for $i \in \{1, 2, \ldots, n\},$ 
\begin{align}
    x_{i+1} = N_i(x_i, \Theta_i),
\end{align}
where $\Theta_i \in \BBR^{l_{\theta_i} \times \ell_i}.$
Note that $x_1 \isdef x.$
The output of the network is finally given by
\begin{align}
    y = S(x_{n+1}) =  \Theta_{n+1}^\rmT x_{n+1},
\end{align}
where $\Theta_{n+1} \in \BBR^{l_{x_{n+1}} \times l_y}.$
The set of neural layer gain matrices $\{ \Theta_i\}_{i=1}^{n+1}$ parameterizes the neural network and is called the \textit{neural network gain}. 

% and the $j$th neuron in $N_i$ is denoted by $n_{ij}.$
% Note that $n_{ij}$ is parameterized by $\theta_{ij} \in \BBR^{l_{\theta_i}},$ where $l_{\theta_i}$ is the number of inputs of $N_i.$







% \clearpage


% Let $l_x = 1$ and $l_y = 1.$ 
% Consider a neural network with two layers with one neuron in each layer. 
% \begin{align}
%     NN(x) 
%         =
%             N_2 (\Theta_2, y)
%         =
%             N_2 (\Theta_2, N_1(\Theta_1, x) )
% \end{align}


% \begin{definition}
%     \rm 
%     A $(n,m)-$\textit{neural layer} is a function $n: \BBR^n \to \BBR^m.$
%     The function $n$ is a composition of a linear function $n_\rml:\BBR^n \to \BBR^m$ and a nonlinearity $n_{\rm nl}:\BBR^{m} \to \BBR^m$. 
%     % Let $x \in \BBR^{l_x}$ be the input to the neuron. 
%     \begin{align}
%         n(x) 
%             = 
%                 n_{\rm nl} (n_\rml (x))
%             % Ax + b
%             =
%                 n_{\rm nl} (A x+ b)
%             =
%                 \sigma (A x+ b).
%     \end{align}
% \end{definition}


% Note that
% \begin{align}
%     \pdt{n}{A} 
%         =
%             \pdt{n}{n_{\rm nl}}
%         =
%             \pdt{n_{\rm nl}}{n_\rml}
%             \pdt{n_\rml}{A}
% \end{align}

==> Sections/UsefulFacts.tex <==
% \subsection{Useful Facts}
The following facts review the well-known results from multivariable calculus. 
\begin{fact}
    \textbf{Derivatives of scalar functions with respect to vectors.}
    Let $a \in \BBR^n,$ $A \in \BBR^{n \times n},$ and $f \colon \BBR^n \to \BBR.$
    Let $x \in \BBR^n$.
    Then, 
    \begin{align}
        \pdt{x^\rmT a}{x}
            &=   
                \pdt{a^\rmT x}{x}
            =   
                a^\rmT \in \BBR^{1 \times n}
            , \\
        \pdt{x^\rmT A x}{x}
            &=   
                2x^\rmT A \in \BBR^{1 \times n},
        \\
        \pdt{f}{x}
            &=   
                \matl 
                    \pdt{f}{x_1} &
                    \cdots &
                    \pdt{f}{x_n} 
                \matr
                 \in \BBR^{1 \times n}.
    \end{align}
\end{fact}
\begin{fact}
    \textbf{Derivatives of vector functions with respect to vectors.}
    Let $A \in \BBR^{m \times n}$ and $f \colon \BBR^n \to \BBR^m.$
    Let $x \in \BBR^n$
    Then, 
    \begin{align}
        \pdt{A x}{x}
            &=   
                A \in \BBR^{m \times n},
        \\
        \pdt{f}{x}
            &=   
                \matl 
                    \pdt{f_1}{x_1} &
                    \cdots &
                    \pdt{f_1}{x_n} 
                    \\ 
                    \vdots & \ddots & \vdots \\
                    \pdt{f_m}{x_1} &
                    \cdots &
                    \pdt{f_m}{x_n} 
                \matr
                 \in \BBR^{m \times n}.
    \end{align}
\end{fact}

\begin{fact}
    \textbf{Derivatives of scalar functions with respect to matrices.}
    Let $a \in \BBR^n,$
    $b \in \BBR^m,$
    $A \in \BBR^{n \times n},$ and
    $f \colon \BBR^{n\times m} \to \BBR.$
    Let $X \in \BBR^{n \times m}$.
    Then, 
    \begin{align}
        \pdt{a^\rmT X b}{X}
            &=   
                b a^\rmT \in \BBR^{m \times n}
            , \\
        \pdt{f}{X}
            &=   
                \matl 
                    \pdt{f}{X_{11}} &
                    \cdots &
                    \pdt{f}{X_{n1}} \\ 
                    \vdots & \ddots & \vdots \\
                    \pdt{f}{X_{1m}} &
                    \cdots &
                    \pdt{f}{X_{mn}} 
                \matr
                 \in \BBR^{m \times n}.
    \end{align}
\end{fact}
% \begin{fact}
%     Useful matrix facts.
%     Let $a,x \in \BBR^n, $ $b \in \BBR^m,$ 
%     $A \in \BBR^{n \times n}$
%     and
%     $B \in \BBR^{m \times n}.$
%     Let $X \in \BBR^{m \times m}.$
%     Then, 
%     \begin{align}
%         \pdt{x^\rmT a}{x}
%             &=   
%                 \pdt{a^\rmT x}{x}
%             =   
%                 a^\rmT \in \BBR^{1 \times n}
%             , \\
%         \pdt{x^\rmT A x}{x}
%             &=   
%                 2x^\rmT A \in \BBR^{1 \times n}
%             , \\
%         \pdt{B x}{x}
%             &=   
%                 B \in \BBR^{m \times n}
%             , \\
%     \end{align}
% \end{fact}

\begin{fact}
    The derivative of the sigmoid function $\sigma(z) = \dfrac{1}{1+e^{-z}}$ is given by
    \begin{align}
        \sigma_z(z)
            \isdef 
        \pdt{\sigma}{z} 
            = 
                \sigma(z) [1-\sigma(z)].
    \end{align}
\end{fact}

\begin{fact}
    \textbf{Chain rule. }
    Let $f \colon \BBR^m \to \BBR^p$ and 
    % $g \colon \BBR^n \to \BBR^m$.
    Define $h \colon \BBR^n \to \BBR^p $ as the composition of $f$ and $g$ , that is, $ f \circ g,$ or, $h(x) = f(g(x)),$ where 
    $x \in \BBR^{n}.$
    Then, 
    \begin{align}
        \pdt{h}{x}
            = 
                \pdt{h}{y} \pdt{y}{x},
    \end{align}
    where $y \isdef g(x) \in \BBR^m.$
    Note that 
    $\pdt{y}{x} \in \BBR^{m \times n}$ and
    $\pdt{h}{y} \in \BBR^{p \times m}$, and thus
    $\pdt{h}{x} \in \BBR^{p \times n}.$
\end{fact}

The following results apply well-known multivariable calculus results to multivariable functions typically used in neural network training. 
\begin{fact}
    Let $x\in \BBR^{l_x}$ and define $\chi \isdef \matl x^\rmT & 1 \matr^\rmT.$
    Then,
    \begin{align}
        \pdt{\chi}{x}
            =
                \SJ_{l_x},
    \end{align}
    where 
    \begin{align}
        \SJ_{l_x} \isdef \matl 
            I_{l_x} \\ 0_{1 \times {l_x} }
        \matr
        \in \BBR^{l_x+1 \times l_x}.
        \label{eq:SJ_def}
    \end{align}
\end{fact}

\begin{fact} 
    Let $z \isdef \SL(x, \theta) = \chi^\rmT \theta,$
    where $\theta \in \BBR^{l_\theta}.$
    Note that $l_\theta = l_x+1.$
    Let $\sigma \colon \BBR \to \BBR.$
    Then, 
    \begin{align}
        \pdt{\sigma(\SL(x, \theta)}{{\theta}}
            &=
                \pdt{\sigma}{{z}}
                \pdt{z}{{\theta}}
            =
                \sigma_z(z)
                \chi^\rmT
            \in \BBR^{ 1 \times l_{\theta}},
     \end{align}
     and
     \begin{align}
        \pdt{\sigma(\SL(x, \theta)}{{x}}
            &=
                \pdt{\sigma}{{z}}
                \pdt{z}{\chi}
                \pdt{{\chi}}{x}
            =
                \sigma_z(z)
                \theta^\rmT 
                \SJ_{l_{x}}
            \in \BBR^{ 1 \times l_{x}}.
    \end{align}
    % 
\end{fact}

\begin{fact} 
    Let $z \isdef \SL(x, \Theta e) = \chi^\rmT \Theta e,$
    where $\Theta \in \BBR^{l_\theta \times \ell}.$
    Note that $e \in \BBR^{\ell}.$
    % 
    Then, 
    \begin{align}
        \pdt{\sigma(\SL(x, \Theta e_j)}{{\Theta}}
            &=
                \pdt{\sigma}{{z}}
                \pdt{z}{{\Theta}}
            =
                \sigma_z(z)
                e
                \chi^\rmT
            \in \BBR^{ \ell \times l_{\theta}}.
    \end{align}
\end{fact}
\vspace{1em}
\begin{fact}
    Let 
    \begin{align}
        N(x,\Theta) 
            =
                \matl
                    \sigma(\SL(x, \Theta e_1) \\
                    \vdots \\
                    \sigma(\SL(x, \Theta e_{\ell})
                \matr
                \in \BBR^{\ell},
    \end{align}
    where
    $\Theta = \matl \theta_1 & \cdots & \theta_\ell \matr \in \BBR^{l_x+1 \times \ell}.$
    Then, for $j=\{1, 2, \ldots, \ell\},$
    \begin{align}
        \pdt{N}{\theta_{j}}
            % =
            %     \pdt{}{\Theta_i}
            %     \matl
            %         \sigma(\SL(x, \Theta_i e_1) \\
            %         \vdots \\
            %         \sigma(\SL(x, \Theta_i e_{\ell_i})
            %     \matr
            &=
                \matl
                    \vdots \\
                    \pdt{\sigma(\SL(x, \theta_{j})}{{\theta_{j}}} \\
                    \vdots \\
                    % \pdt{\sigma(\SL(x_i, \theta_{i \ell_i} )}{{\theta_{ij}}}
                \matr
            % =
            %     \matl
            %         \vdots \\
            %         \sigma(z_{ij})
            %         \left( 1 - \sigma(z_{ij}) \right)
            %         x_i^\rmT \\
            %         \vdots
            %     \matr
            =
                \sigma_z(z_{j}) 
                % \left( 1 - \sigma(z_{ij}) \right) 
                e_j \chi^\rmT
                \in \BBR^{\ell \times l_{\theta}}
                ,
        \\
        \pdt{N}{x}
            &=
                \matl
                    \vdots \\
                    \pdt{\sigma(\SL(x, \theta_j)}{{x}} \\
                    \vdots
                \matr
            =
                \matl
                    \vdots \\
                    \sigma_z(z_{j})
                    % e_j^\rmT \Theta ^\rmT 
                    \theta_j^\rmT
                    \SJ_{l_x} \\
                    \vdots
                \matr
            \nn \\ &
            =
                \Lambda(x, \Theta) \Theta^\rmT \SJ_{l_x}
                \in \BBR^{\ell \times l_{x}  }
                ,
    \end{align}
    where 
    \begin{align}
        \Lambda(x, \Theta)
            =
                {\rm diag \ }
                (
                    \sigma_z(\SL(x, \theta_1)),
                    \ldots,
                    \sigma_z(\SL(x, \theta_\ell))
                )
            \in \BBR^{\ell \times \ell}.
        \label{eq:Lambda_def}
    \end{align}
\end{fact}
% \vspace{2em}



\begin{fact}
    \textbf{Backpropagation.}
    \label{fact:dy/dtheta}
    % Let $\theta_{ij} \in \BBR^{l_{\theta_i}} $ denote the $j$th column of $\Theta_i.$
    % Note that $\theta_{ij} =\Theta_i e_j,$ where $j \in \{1,2,\ldots, \ell_i\}.$
    Let $z_{ij} = \SL(x_i, \Theta_i e_j).$
    Then, for $i<n+1,$
    \begin{align}
        \pdt{y}{\theta_{ij}}
            &=
                \Theta_{n+1}^\rmT
                \prod_{q=n}^{i+1}
                \Lambda(x_{q}, \Theta_{q}) \Theta_{q}^\rmT \SJ_{l_{x_q}}
                \sigma_z(z_{ij}) e_j x_i^\rmT,
    \end{align}
    where $e_j$ is the $j$th column of the $\ell_i\times \ell_i$ identity matrix. 
    % 
    Furthermore, for $i=n+1,$
    \begin{align}
        \pdt{y}{\theta_{n+1,j}}
            &=
                \pdt{\Theta_{n+1}^\rmT x_{n+1}}{\theta_{n+1,j}}
            % =
            %     \pdt{}{\theta_{n+1,j}}
            %     \matl
            %         \vdots \\
            %         \theta_{n+1,j}^\rmT x_{n+1} \\
            %         \vdots
            %     \matr
            % \nn \\
            % &=
            %     \matl
            %         \vdots \\
            %         x_{n+1}^\rmT  \\
            %         \vdots \\
            %     \matr
            =
                e_j x_{n+1}^\rmT.
    \end{align}
    
\end{fact}

\begin{proof}
    Note that, for $i<n+1,$
    \begin{align}
        \pdt{y}{\theta_{ij}}
            &=
                % \pdt{\Theta_{n+1}^\rmT x_{n+1}}{\theta_{ij}}
                \pdt{S(x_{n+1})}{\theta_{ij}}
                % \pdt{N_n}{x_n}
            \nn \\
            &=
                \pdt{S(x_{n+1})}{x_{n+1}}
                \pdt{x_{n+1}}{\theta_{ij}}
            \nn \\
            &=
                \Theta_{n+1}^\rmT
                \pdt{N_n(x_{n},\Theta_n)}{\theta_{ij}}
            \nn \\
            &=
                \Theta_{n+1}^\rmT
                \pdt{N_n(x_{n},\Theta_n)}{x_n}
                \pdt{x_n}{\theta_{ij}}
            \nn \\
            &=
                \Theta_{n+1}^\rmT
                \Lambda(x_n, \Theta_n) \Theta_n^\rmT \SJ_{l_{x_n}}
                \pdt{N_{n-1}(x_{n-1},\Theta_{n-1})}{\theta_{ij}}
            \nn \\
            &=
                \Theta_{n+1}^\rmT
                \Lambda(x_n, \Theta_n) \Theta_n^\rmT \SJ_{l_{x_n}}
                \Lambda(x_{n-1}, \Theta_{n-1}) 
                \nn \\ &\quad 
                \cdot \Theta_{n-1}^\rmT \SJ_{l_{x_{n-1}}}
                \pdt{N_{n-2}(x_{n-2},\Theta_{n-2})}{\theta_{ij}}
            \nn \\
            &=
                \Theta_{n+1}^\rmT
                \prod_{q=n}^{i+1}
                \Lambda(x_{q}, \Theta_{q}) \Theta_{q}^\rmT \SJ_{l_{x_q}}
                \pdt{N_{i}(x_{i},\Theta_{i})}{\theta_{ij}}
            \nn \\
            &=
                \Theta_{n+1}^\rmT
                \prod_{q=n}^{i+1}
                \Lambda(x_{q}, \Theta_{q}) \Theta_{q}^\rmT \SJ_{l_{x_q}}
                \sigma_z(z_{ij}) e_j x_i^\rmT. \nn 
    \end{align}
\end{proof}

% \begin{fact} 
%     % \textbf{Useful facts. }
%     Let $x_i \in \BBR^{l_{x_i}},$ which implies that $\chi \in \BBR^{l_{\theta_i}},$ where $l_{\theta_i} \isdef l_{x_i}+1.$
%     % be the sigmoid function. 
%     Let $z_{ij} \isdef \SL(x_i, \Theta_i e_j) = \chi_i^\rmT \Theta_i e_j.$
%     Let $\sigma \colon \BBR \to \BBR.$
%     Then, 
%     \begin{align}
%         \pdt{\sigma(\SL(x_i, \Theta_i e_j)}{{\Theta_i}}
%             &=
%                 \pdt{\sigma}{{z_{ij}}}
%                 \pdt{z_{ij}}{{\Theta_i}}
%             =
%                 \sigma_z(z_{ij})
%                 e_j \chi_i^\rmT,
%             \in \BBR^{ \ell_i \times l_{\theta_i}},
%         \\
%         \pdt{\sigma(\SL(x_i, \Theta_i e_j)}{{x_i}}
%             &=
%                 \pdt{\sigma}{{z_{ij}}}
%                 \pdt{z_{ij}}{{\chi_i}}
%                 \pdt{{\chi_i}}{x_i}
%             =
%                 \sigma_z(z_{ij})
%                 e_j^\rmT \Theta_i^\rmT 
%                 \SJ_{l_{x_i}},
%             \in \BBR^{ 1 \times l_{\theta_i}},
%     \end{align}
%     where 
%     Furthermore, 
%     \begin{align}
%         % \pdt{N_i}{\Theta_i}
%         %     % =
%         %     %     \pdt{}{\Theta_i}
%         %     %     \matl
%         %     %         \sigma(\SL(x, \Theta_i e_1) \\
%         %     %         \vdots \\
%         %     %         \sigma(\SL(x, \Theta_i e_{\ell_i})
%         %     %     \matr
%         %     &=
%         %         \matl
%         %             \pdt{\sigma(\SL(x, \Theta_i e_1)}{{\Theta_i}} \\
%         %             \vdots \\
%         %             \pdt{\sigma(\SL(x, \Theta_i e_{\ell_i})}{{\Theta_i}}
%         %             % \sigma(\SL(x, \Theta_i e_{\ell_i})
%         %         \matr
%         %     =
%         %         \matl
%         %             \sigma(z_{i1})
%         %             \left( 1 - \sigma(z_{i1}) \right)
%         %             x_i e_1^\rmT \\
%         %             \vdots \\
%         %             \sigma(z_{i\ell_i})
%         %             \left( 1 - \sigma(z_{i\ell_i}) \right)
%         %             x_i e_{\ell_i}^\rmT
%         %             % \sigma(\SL(x, \Theta_i e_{\ell_i})
%         %         \matr
%         %         \in \BBR^{l_{\theta_i} \ell_i \times \ell_i}
%         %         ,
%         % \\
%         % \\
%         \pdt{N_i}{x_i}
%             % =
%             %     \pdt{}{x_i}
%             %     \matl
%             %         \sigma(\SL(x, \Theta_i e_1) \\
%             %         \vdots \\
%             %         \sigma(\SL(x, \Theta_i e_{\ell_i})
%             %     \matr
%             &=
%                 \matl
%                     \pdt{\sigma(\SL(x_i, \Theta_i e_1)}{{x_i}} \\
%                     \vdots \\
%                     \pdt{\sigma(\SL(x_i, \Theta_i e_{\ell_i})}{{x_i}}
%                     % \sigma(\SL(x, \Theta_i e_{\ell_i})
%                 \matr
%             =
%                 \matl
%                     \sigma_z(z_{i1})
%                     % \left( 1 - \sigma(z_{i1}) \right)
%                     e_1^\rmT \Theta_i ^\rmT \\
%                     \vdots \\
%                     \sigma_z(z_{i\ell_i})
%                     % \left( 1 - \sigma(z_{i\ell_i}) \right)
%                     e_{\ell_i}^\rmT \Theta_i^\rmT
%                     % \sigma(\SL(x, \Theta_i e_{\ell_i})
%                 \matr
%             =
%                 \Lambda(x_i, \Theta_i) \Theta_i^\rmT
%                 \in \BBR^{\ell_i \times l_{\theta_i}  }
%                 ,
%     \end{align}
%     where 
%     \begin{align}
%         \Lambda(x_i, \Theta_i)
%             =
%                 {\rm diag \ }
%                 (
%                     \sigma_z(z_{i1}),
%                     \ldots,
%                     \sigma_z(z_{i\ell_i})
%                 )
%                 % \matl
%                 %     \sigma_z(z_{i1})
%                 %     \\
%                 %     \vdots \\
%                 %     \sigma_z(z_{i\ell_i})
%                 %     % \left( 1 - \sigma(z_{i\ell_i}) \right)
%                 % \matr
%             \in \BBR^{\ell_i \times \ell_i}.
%     \end{align}
%     and
%     \begin{align}
%         \pdt{N_i}{\theta_{ij}}
%             % =
%             %     \pdt{}{\Theta_i}
%             %     \matl
%             %         \sigma(\SL(x, \Theta_i e_1) \\
%             %         \vdots \\
%             %         \sigma(\SL(x, \Theta_i e_{\ell_i})
%             %     \matr
%             &=
%                 \matl
%                     \vdots \\
%                     \pdt{\sigma(\SL(x_i, \theta_{ij})}{{\theta_{ij}}} \\
%                     \vdots \\
%                     % \pdt{\sigma(\SL(x_i, \theta_{i \ell_i} )}{{\theta_{ij}}}
%                 \matr
%             % =
%             %     \matl
%             %         \vdots \\
%             %         \sigma(z_{ij})
%             %         \left( 1 - \sigma(z_{ij}) \right)
%             %         x_i^\rmT \\
%             %         \vdots
%             %     \matr
%             =
%                 \sigma_z(z_{ij}) 
%                 % \left( 1 - \sigma(z_{ij}) \right) 
%                 e_j x_i^\rmT
%                 \in \BBR^{\ell_i \times l_{\theta_i}}
%                 ,
%     \end{align}
% \end{fact}
